Constraints on neutrino masses from Lyman-alpha forest power spectrum with BOSS and XQ-100

We present constraints on masses of active and sterile neutrinos. We use the one-dimensional Ly$\alpha$-forest power spectrum from the Baryon Oscillation Spectroscopic Survey (BOSS) of the Sloan Digital Sky Survey (SDSS-III) and from the VLT/XSHOOTER legacy survey (XQ-100). In this paper, we present our own measurement of the power spectrum with the publicly released XQ-100 quasar spectra. Fitting Ly$\alpha$ data alone leads to cosmological parameters in excellent agreement with the values derived independently from Planck 2015 Cosmic Microwave Background (CMB) data. Combining BOSS and XQ-100 Ly$\alpha$ power spectra, we constrain the sum of neutrino masses to $\sum m_\nu < 0.8$ eV (95\% C.L). With the addition of CMB data, this bound is tightened to $\sum m_\nu < 0.14$ eV (95\% C.L.). With their sensitivity to small scales, Ly$\alpha$ data are ideal to constrain $\Lambda$WDM models. Using XQ-100 alone, we issue lower bounds on pure dark matter particles: $m_X \gtrsim 2.08 \: \rm{keV}$ (95\% C.L.) for early decoupled thermal relics, and $m_s \gtrsim 10.2 \: \rm{keV}$ (95\% C.L.) for non-resonantly produced right-handed neutrinos. Combining the 1D Ly$\alpha$ forest power spectrum measured by BOSS and XQ-100, we improve the two bounds to $m_X \gtrsim 4.17 \: \rm{keV}$ and $m_s \gtrsim 25.0 \: \rm{keV}$ (95\% C.L.). The $3~\sigma$ bound shows a more significant improvement, increasing from $m_X \gtrsim 2.74 \: \rm{keV}$ for BOSS alone to $m_X \gtrsim 3.10 \: \rm{keV}$ for the combined BOSS+XQ-100 data set. Finally, we include in our analysis the first two redshift bins ($z=4.2$ and $z=4.6$) of the power spectrum measured with the high-resolution HIRES/MIKE spectrographs. The addition of HIRES/MIKE power spectrum allows us to further improve the two limits to $m_X \gtrsim 4.65 \: \rm{keV}$ and $m_s \gtrsim 28.8 \: \rm{keV}$ (95\% C.L.).

==> data.tex <==
\begin{figure}[htbp]
\begin{center}
\epsfig{figure= plots/PkBOSS.pdf,width = 7.5cm}
\epsfig{figure= plots/PkXQ100.pdf,width = 7.5cm}
\caption{\it Left plot: 1D Ly$\alpha$ forest power spectrum from the SDSS-III/BOSS DR9 data. Right plot: 1D Ly$\alpha$ forest power spectrum from the XQ-100 data . The solid curves show the best-fit model when considering Ly$\alpha$ data alone.  The oscillations  arise  from Ly$\alpha$-Si\,III correlations, which occur at a  wavelength separation $\Delta \lambda = 9.2$\AA.} 
\label{fig:P1D}
\end{center}
\end{figure}

